Scaling laws for concentration-gradient-driven electrolyte transport through a 2D membrane

Two-dimensional (2D) nanomaterials exhibit unique properties that are promising for diverse applications, including those relevant to concentration-gradient-driven transport of electrolyte solutions through porous membranes made from these materials, such as water desalination, osmotic power, and iontronics. Here we derive general equations, and determine scaling laws in the thick and thin electric-double-layer limits, that quantify the variation of the concentration-gradient-driven flow rate, solute flux and electric current with the pore radius, surface charge density and Debye screening length for the transport of a dilute electrolyte solution through a circular aperture in an infinitesimally thin planar membrane. We also determine scaling laws for the electric-field-driven flow rate in the thin electric-double-layer limit in the same geometry. We show that these scaling laws accurately capture the scaling relationships from finite-element numerical simulations within the Debye-H\"uckel regime, and extend the theory to obtain scaling laws in the thin electric-double-layer limit that hold even when the electric potential energy is large compared with the thermal energy. These scaling laws indicate unusual behavior for concentration-gradient-driven flow in a 2D membrane that is not seen in thicker membranes, which has broad implications for liquid transport through membranes whose thickness comparable to, or smaller than, their pore size.

==> 2D_membrane_CDF-paper-aux.tex <==



==> 2D_membrane_CDF-sm-aux.tex <==


